Correctness by construction for probabilistic programs

The "correct by construction" paradigm is an important component of modern Formal Methods, and here we use the probabilistic Guarded-Command Language $\mathit{pGCL}$ to illustrate its application to $\mathit{probabilistic}$ programming. $\mathit{pGCL}$ extends Dijkstra's guarded-command language $\mathit{GCL}$ with probabilistic choice, and is equipped with a correctness-preserving refinement relation $(\sqsubseteq)$ that enables compact, abstract specifications of probabilistic properties to be transformed gradually to concrete, executable code by applying mathematical insights in a systematic and layered way. Characteristically for "correctness by construction", as far as possible the reasoning in each refinement-step layer does not depend on earlier layers, and does not affect later ones. We demonstrate the technique by deriving a fair-coin implementation of any given discrete probability distribution. In the special case of simulating a fair die, our correct-by-construction algorithm turns out to be "within spitting distance" of Knuth and Yao's optimal solution.

==> ISoLA to arXiv 200730/ISoLA-Morgan-Macros.tex <==
%% For TeXshop: make it LaTeX the root file if you cmt-T here.
%% !TEX root = ISoLA.tex 
%

\newcommand\BB[1]{{\color{blue}#1}}
\newcommand\RR[1]{{\color{red}#1}}
\newcommand\OZ[1]{1\;\PC{\PF#1}\;0}
\newcommand\CalX {{\ensuremath{\cal X}}}
\newcommand\Body {\Meta{Body}}
\newcommand\Spec {\Meta{Spec}}
\newcommand\Imp {\Meta{Imp}}
\newcommand\Left {\Meta{Left}}
\newcommand\Right {\Meta{Right}}
\newcommand\Prog {\Meta{Prog}}
\newcommand\Prop {\Meta{prop}}
\newcommand\Pre {\Meta{pre}}
\newcommand\Post {\Meta{post}}
\newcommand\pGCL {\textit{pGCL}}
\newcommand\Exp {\Meta{E}}
\newcommand\Cond {\Meta{C}}
\newcommand\Sbst[3]{#1[#2\ensuremath\backslash#3]}
\newcommand\B {\kern.12em\raisebox{.5ex}{\framebox[.35em]{\rule{0pt}{.5ex}}}\kern.47em}
\newcommand\Ass[1] {\ensuremath{\color{blue}\left\{\,{\PF{#1}}\,\right\}}}
\newcommand\Qdot {\HangRight{\textrm{\quad.}}}
\newcommand\Qcomma {\HangRight{\textrm{\quad,}}}
\newcommand\AST {\textit{AST}}
\newcommand\In {:\kern-.1em$\in$\kern-.2em}
\newcommand\St {:\kern-.1em$|$\kern-.2em}
\newcommand\CbC {\textit{C\kern.03emb\kern-.045emC}}
\newcommand\Footnote[1] {\footnote{{\color{red}\sf#1}}}
\newcommand\Cite[1] {{\color{red}\sf[#1]}}

\newcommand\Itm[1] {(\ref{#1})}
%\newcommand\Secs[1] {\S\S#1}
\newcommand\Secs[1] {Secs.~\ref{#1}}
%\newcommand\Sec[1] {\S\kern.03em\ref{#1}}
\newcommand\Sec[1] {Sec.~\ref{#1}}
\newcommand\Union		{\mathbin{\cup}}
\newcommand\Ref			{\mathrel\sqsubseteq}
\newcommand\Prg[1] {Program\,(\ref{#1})}
\newcommand\LHS			{\textit{lhs}}
\newcommand\RHS			{\textit{rhs}}
\newcommand\Supp[1]	{\ensuremath{\lceil#1\rceil}} % Support of a distribution.
\newcommand\Dist {\ensuremath{\mathbb D}}
\newcommand\Pow			{{\mathbb P}}%\kern-.05em}
\newcommand\FF {\NF{1}{2}} % Shortcut: "fifty-fifty".			
\newcommand\Min {\ensuremath{\mathbin{\sf min}}}
\newcommand\WP {\textsf{wp}}
\newcommand\WPP[2] {\WP(\texttt{#1},#2)}
\newcommand\False {\ensuremath{\mathit{False}}}
\newcommand\True {\ensuremath{\mathit{True}}}
\newcommand\Meta[1] {{\texttt{\textit{#1}}}}
\newcommand\HangRight[1]	{\makebox[0pt][l]{#1}}
\newcommand\HangLeft[1]		{\makebox[0pt][r]{#1}}
\newcommand\Implies		{\mathbin{\Rightarrow}} % Proper spacing for binary operator.
\newcommand\ND			{\ensuremath{\mathbin{\sqcap}}}
\newcommand\NF[2]		{\ensuremath{\nicefrac{#1}{#2}}} % Abbreviation.
\newcommand\NSF[2]		{\ensuremath{\nicefrac{#1\,}{\,#2}}} % Abbreviation; add some space.
\newcommand\PC[1]		{\ensuremath{\mathbin{{}_{{#1}}\kern-.05em\oplus}}}
\newcommand\PPC[2]		{\ensuremath{\mathbin{{}_{{#1}}\kern-.05em\oplus_{{#2}}}}}
\newcommand\PCF			{\PCNF{1}{2}}
\newcommand\PCNF[2]		{\PC{\NF{#1}{#2}}}
\newcommand\PF[1][\empty]	{\ifx\empty#1\empty\tt\else\texttt{#1}\fi} % Program font: \PF sets it; \PF[x] applies it.
\newcommand\Wide[1] 		{~~~#1~~~} % Basic space.
\newcommand\WIDERM[1]	{\Wide{\WideRm{#1}}} % Extra wide space around text.
\newcommand\WideRm[1]	{~~~\textrm{#1}~~~} % Basic space, but around text.

\newcommand\Eqn[1] {(\ref{#1})}
\newcommand\Fig[2][\empty] {\ifx#1\empty Fig.~\ref{#2}\else Fig.~\ref{#2}(#1)\fi}
\newcommand\ProgIL[1] {~\texttt{#1}~}

\newenvironment{ProgEqn}[1][]
	{\def\L{#1}\ifx\L\empty\[\else\begin{equation}\label{#1}\fi%
		\begin{minipage}{.8\linewidth}\texttt\bgroup%
			\vspace*{-2.5ex} % tabbing introduces unwanted vertical space.
			\begin{tabbing}
				\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
				\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
				\quad\=
			\kill}
	{\end{tabbing}\egroup\end{minipage}\ifx\L\empty\]\else\end{equation}\fi}
						
%\newenvironment{ZZProgEqn}[1][]
%	{\def\L{#1}\ifx\L\empty
%	empty
%%		\begin{tabbing}\tt
%%			\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%%			\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%%			\quad\=\+\+
%%			\kill
%	\else
%non-empty
%%	\begin{equation}\label{#1}%
%%		\begin{minipage}{.8\linewidth}
%%			\begin{tabbing}\tt
%%				\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%%				\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%%				\quad\+\+
%%				\kill
%%			\end{tabbing}
%%		\end{minipage}
%%	\end{equation}
%	\fi}
%	{\ifx\L\empty
%EMPTY
%%	\end{tabbing}
%	\else
%NON-EMPTY	
%%		\end{tabbing}\end{minipage}\end{equation}
%	\fi}
			
%\newenvironment{ProgEqn}{\tt
%	\begin{tabbing}
%		\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%		\quad\=\quad\=\quad\=\quad\=\quad\=\quad\=
%		\quad\=\+\+
%		\kill
%	}{\end{tabbing}}
	
\newcommand\Com {\`\footnotesize\sf--~} % Comment for ProgMini, right-adjusted.
\newcommand\LCom {\footnotesize\sf--~} % Comment for ProgMini, at left.


\newenvironment{Reason}{\begin{tabbing}\hspace{4em}\= \hspace{1cm} \= \kill}
{\end{tabbing}\vspace{-1em}}
\newcommand\Step[2] {#1 \> $\begin{array}[t]{@{}llll}#2\end{array}$ \\}
\newcommand\StepR[3] {#1 \> $\begin{array}[t]{@{}llll}#3\end{array}$
\` {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\WideStepR[3] {#1 \>
$\begin{array}[t]{@{}ll}~\\#3\end{array}$ \`
{\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\Space {~ \\}
\newcommand\RF {\small}

\newenvironment{Refines}{\begin{list}{$\Ref$}{
\setlength{\rightmargin}{0em}
\addtolength{\leftmargin}{1em}
\setlength{\listparindent}{0em}
\setlength{\labelwidth}{2em}}}{
\end{list}}
\newcommand\Unspace {\vspace{-1.4ex}}

\newcommand\PStep[2] {$#1$ \> {\PF \begin{tabular}[t]{@{}llll}#2\end{tabular}} \\}
\newcommand\PStepR[3] {$#1$ \>  {\PF \begin{tabular}[t]{@{}llll}#3\end{tabular}}
\` {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\WidePStepR[3] {$#1$ \>
{\PF \begin{tabular}[t]{@{}llll}#3\end{tabular}} \`
{\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}

%%%% MacrosMaths 24 September 2016. 
%%%% Have not bothered to sort them into sections, because it's too hard to manage duplication between authors.
%%%% Instead, it's one long list that can be sorted and then checked for duplicates.
%
%%%% Please be careful not to (let your editor) accidentally replace the tabs by spaces.
%
%%%% DON'T SEE YOUR MACRO HERE?
%%%% It might be in the commented-out section at the end: just uncomment and move into the main part.
%%%% All the ones that are here are actually being used by somebody somewhere (I think).
%
%
%% \newcommand\ABC[1]		{\ACapty{#1}{\GId}{\AllPi}}  % Additive Bayes Capacity
%\newcommand\ABC[1]		{\ACapty{#1}{1}{\AllPi}}  % Additive Bayes Capacity Carroll 180906
%\newcommand\Abort			{\fbox{DEPRECATED}}		% Abort command
%\newcommand\Abs[1]		{\ensuremath{#1}}		% Abstract channel
%\newcommand\AHSpc 		{\Dist\calx{\Fun}\,\Dist^2\calx} % The "raw" denotational space of forward HMM's.
%\newcommand\ACapty[3]		{\calml^+_{#2}(#3,#1)} % additive capacity
%\newcommand\AllPi			{{\Dist}} % symbol used for "maximize over pi" in capacities
%\newcommand\App[1]		{App.~\ref{#1}}
%\newcommand\AT			{@} % For `` with probability''.
%\newcommand\Atm			{\mathbin{\ast}}	% Arithmetic times.
%\newcommand\Ato[1]		{^{@#1}} % Probability of element in distribution enumeration.
%\newcommand\Att[2]			{^{@\nicefrac{#1}{#2}}} % Probability of element in distribution enumeration.
%\newcommand\Avg 			{{\sf avg}}
%\newcommand\AVG 			{\mathop\mu}
%%\newcommand\BayesLeak	{\call_{\GId}} % Bayes-leakage, so that we can drop or not the g_id 1020.
%\newcommand\BayesLeak	{\call_1} % Bayes-leakage, so that we can drop or not the g_id 1020. CCM 180906
%% \newcommand\Begin		{\tt|[} % Open local-declaration scope.
%\newcommand\Begin			{\PF[\{]} % Open local-declaration scope.
%\newcommand\Bool		{\mathit{Bool}}
%\newcommand\BV[1][1]		{V_{#1}} % 1020.
%\newcommand\cala		{\mathcal{A}}	% Adversary
%\newcommand\calb		{\mathcal{B}}	% Adversary
%\newcommand\calc		{\mathcal{C}}	% Adversary
%\newcommand\cald		{\mathcal{D}}	% Set of priors
%\newcommand\cale		{\mathcal{E}}	% Set of electors
%\newcommand\calg		{\mathcal{G}}	% Subset of gain functions
%\newcommand\calh		{\mathcal{H}}	% Hidden variables
%\newcommand\call		{\mathcal{L}}	% Leakage
%\newcommand\calml		{\mathcal{M\kern-.15emL}}	% Capacity symbol
%\newcommand\calo		{\mathcal O} % Outcome of an election.
%\newcommand\calp		{\mathcal{P}}	% Programs
%\newcommand\cals		{\mathcal{S}}	% Subset of secret values
%\newcommand\calu		{\mathcal{U}}	% Collection of sets
%\newcommand\calv		{\mathcal{V}}	% Visible variables
%\newcommand\calw		{\Spc{W}}	% Space of actions
%\newcommand\calx		{\Spc{X}}	% Space of hidden inputs
%\newcommand\caly		{\Spc{Y}}	% Space of observable outputs
%\newcommand\calz		{\Spc{Z}}	% Another space of observable outputs
%\newcommand\calf		{\Spc{F}}	% Space of functions
%\newcommand\calk		{\Spc{K}}	% Mechanism to sanitize queries in statistical databases
%\newcommand\Caption[1] {\caption{\protect\makebox[0pt][r]{---\hspace{6em}}#1\protect\makebox[0pt][l]{\hspace{1em}---}}}
%\newcommand\CC 		{\mbox{\boldmath$\cal C$}} % Contexts.
%\newcommand\CCC		{{\mathbb C}} % Set of contexts.
%\newcommand\CP		{\times} % Cartesian product
%\newcommand\CComp		{\mathbin{\parallel}}
%\newcommand\CEqv			{\mathrel{\equiv}} % Two channel matrices are eqivalent.
%\newcommand\Ch			{\Conc{C}}
%\newcommand\ChanHyp[2]	{\MakeHyp{\Joint{#1}{#2}}} % Now replaced by just \Hyp.
%\newcommand\ChApp[2]		{#1{\rhd}#2}
%\newcommand\Chi 			{\raisebox{.15em}{$\chi$}}
%\newcommand\CId			{C_{\textnormal{id}}} % transparent channel (identity matrix)
%\newcommand\CloseSem		{]\kern-.16em]}
%\newcommand\Comma 		{\quad\textrm{,}} % For end of program displays.
%\newcommand\Comp		{\mathbin{\circ}} % Functional composition.
%\newcommand\Conc[1]		{\textnormal{\textsf{#1}}}	% Concrete channel
%\newcommand\CONC[1]		{\mbox{\fontfamily{lmss}\selectfont#1}} % Use this for G so that it's not confused with C.
%\newcommand\Cond[3]		{#1\lhd#2\rhd#3} % Conditional
%\newcommand\Consonant {\textsf{Consonant}}
%\newcommand\CT[3]			{$\Conc{#1}{\In}\csname cal#2\endcsname{\MFun}\csname cal#3\endcsname$} % Channel with type.
%\newcommand\CVec[1]		{(#1)}
%\newcommand\dbitem		{\mathrm{x}}	% sequences of elements in statistical databases
%\newcommand\DE[1]			{\DistEnum{#1}} % Shortcut.
%\newcommand\Defs			{{:=}\,}
%\newcommand\DELTA		{\underline{\Delta}}
%\newcommand\Dem[1]		{#1^\sqcap}
%\newcommand\DemRef		{\mathrel{\Ref_\sqcap}}
%%\newcommand\Diag[1]	{\Conc{D}^{#1}}
%%\newcommand\Diag[1]	{\raisebox{.55ex}{\fbox{\raisebox{0ex}[.5ex][0ex]{\makebox[.1em][c]{\scriptsize$#1$}}}}}
%\newcommand\DiagB[1]		{\lceil\kern-.16em#1\kern-.14em\rfloor} % Annabelle likes this one.
%\newcommand\Diag[1]		{\raisebox{.4ex}{$\ulcorner\kern-.3em#1\kern-.3em\raisebox{-.5ex}{$\lrcorner$}$}}
%\newcommand\DTrial[1]	{\lceil\kern-.1em#1\kern-.13em\rfloor}
%\newcommand\Dist			{{\mathbb D}}
%\newcommand\DistA[1]		{{\mathbb D}{#1}} % With an argument.
%\newcommand\DistEnum[1]	{[#1]}
%\newcommand\DKL			{D_{\mathit{KL}}}
%\renewcommand\Dot 			{\quad\textrm{.}} % For end of program displays.
%\newcommand\DSet[1]		{\{#1\}}
%\newcommand\DU			{\mathbin{\uplus}} % Disjoint union.
%%\newcommand\End		{{\tt]|}} % Close local-declaration scope.
%\newcommand\Early {\textsf{Early}}
%\newcommand\Else {\textbf{else}}
%\newcommand\EN			{$-$} % For en-dash between words. Existing one is too thin.
%\newcommand\End			{\PF[\}]} % Close local-declaration scope.
%\newcommand\EQV			{eqv.}
%\newcommand\Expec[2]		{{\cal E}_{#1}{#2}} % Expected value.
%\newcommand\Expt[2]		{{\cal E}_{#1}\,#2} % Expected value with kern.
%\newcommand\ExtPC[1]		{\mathbin{{}_{#1}\kern-.15em+\kern-.75em+}}
%\newcommand\False			{\mbox{\it false}} % {\textit{false}}
%\newcommand\From 		{\mbox{\rm :\kern-.1em$\in$}} % Introduction of new name, with type.
%\newcommand\Fun			{\mathbin{\rightarrow}} % Make it an operator to get correct spacing.
%
%% classes of gain functions
%\newcommand\GainFunc[1]		{{\mathbb G}#1} % By analogy with other type-condstructors like \Dist.
%\newcommand\GainFin[1]		{\GainFunc^{\textnormal{fin}}\kern-.1em{#1}} % finite actions
%\newcommand\GainNN[1]		{\GainFunc^+\kern-.2em{#1}} % non-negative gain functions
%\newcommand\GainOneSpan[1]	{\GainFunc^{1}{#1}} % 1-spanning gain functions
%\newcommand\GainOneSpanVg[1]{\GainFunc^{\UpDownStr}{#1}} % g giving 1-spanning V_g
%
%% gain functions
%\newcommand\GHappy		{g_{\smiley}}
%\newcommand\GSad		{g_{\frownie}}
%\newcommand\GId			{g_{\textnormal{id}}}
%\newcommand\GTiger		{g_{\kern0.05em\textnormal{tiger}}}
%\newcommand\GLion		{g_{\textnormal{\,lion}}}
%\newcommand\GGates		{g_{\kern0.05em\textnormal{Gates}}}
%\newcommand\GRecip[1]	{g_{#1^{\text{--}1}}} % reciprocals of pi gain function
%\newcommand\GShift[2][g]{{#1}_{+ #2}} % shifted gain function
%\newcommand\GScale[2][g]{{#1}_{\times #2}} % scaled gain function
%\newcommand\GCompl[1]	{{#1^c}} % complement of gain function
%
%\newcommand\Gets			{{:=}\,}
%\newcommand\Heads		{\textit{heads}}
%\newcommand\HMM			{\textit{HMM}}
%\newcommand\HMMConc[2]	{(\Conc{#1}{;}\Conc{#2})}
%\newcommand\HMMone[1]	{\OpenSem#1\CloseSem}
%\newcommand\HMMsem[2]	{\OpenSem#1{:}#2\CloseSem}
%\newcommand\Hyp[2]		{\MakeHyp{\Joint{#1}{#2}}} % Replaces \ChanHyp.
%\newcommand\HypA[1]		{{\mathbb D}^2{#1}} % Type, with an argument.
%%\newcommand\HypT			{{\mathbb H}} % Type, without an argument.
%\newcommand\HypT			{{\mathbb D}^2} % Type, without an argument.
%\newcommand\ID			{{\sf id}}
%%\newcommand\Id[1]		{\textsf{Id}_{#1}} % Doesn't seem to be used.
%\newcommand\Id			{\Conc{I}}
%\newcommand\If {\textbf{if}}
%\newcommand\In			{{:}\,} % Careful spacing for ":" meaning "is of type".
%\newcommand\ind			{\Spc{I}}	% indes of indviduals in statistical databases
%\newcommand\Input			{\mbox{$\cal I$}} % Channel input.
%\newcommand\InQuadL[1] {\makebox[0pt][l]{$#1$}\quad}
%\newcommand\Inter			{\mathbin{\cap}}
%\newcommand\ITE[3]		{(\textrm{$#1$ if $#2$ else $#3$})} % IF-THEN-ELSE expression
%% \newcommand\Joint[2]		{#1\rangle#2}
%\newcommand\Joint[2]		{#1{\kern-0.6pt\smalltriangleright\kern.3pt}#2} % needs hack (below) to get \smalltriangleright from mathabx without loading it
%\newcommand\Knows		{\textsf{K}}
%%\newcommand\Leak 			{\PF[\tt{\textbf{pr\i nt}}]} % 1159: Get font right! Use dotless i so we know it's a macro. We can change its definition later.
%%\newcommand\Leak 			{\PF[\tt{\textbf{leak}}]} % Now trying this out 180513.
%\newcommand\Late			{\textsf{Late}}
%\newcommand\Leak 			{\PF[PRINT]} % Now trying this out 180522.
%\newcommand\LeakGeq		{\geq_{\GainFunc{}}}	% leakage order
%\newcommand\LeakNotGeq	{\not\geq_{\GainFunc{}}}	% (not) leakage order
%\newcommand\LMat[3] {\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\left(\rule{0pt}{#3}\right.\hspace{#1}$}}}
%\newcommand\LossFunc[1]		{{\mathbb L}#1}
%\newcommand\LowVar		{{\tt lowvar}}	%  Declaration of low-securty (possibly local) variable.
%%\newcommand\mbc[1]		{\mathcal{M}\!\mathcal{L}^\times\!(#1)}  % Multiplicative Bayes Capacity
%%\newcommand\mbc[1]		{\MCapty{#1}{\GId}{\AllPi}}  % Multiplicative Bayes Capacity
%\newcommand\mbc[1]		{\MCapty{#1}{1}{\AllPi}}  % Multiplicative Bayes Capacity Carroll 180906
%\newcommand\MakeHyp[1]	{[#1]}
%\newcommand{\MCap}		{{\cal M}}
%\newcommand\MCapty[3]		{\calml^{\times}_{#2}(#3,#1)} % multiplicative capacity
%\newcommand\Meet			{\mathrel{\sqcap}}
%\newcommand\Metric			{{\mathbb M}}
%\newcommand\MFun			{\mathbin{\rightarrowtriangle}}
%\newcommand\MH			{\calx{\MFun}\caly{\times}\calx} % Matrix-H.
%\newcommand\Min			{\mathbin\textsf{min}}
%\newcommand\MinArg		{\mathbin\textsf{minarg}}
%\newcommand\MMult		{\mathbin{\cdot}} % Matrix multiplication.
%\newcommand\Mod			{\mathbin{\rm mod}}
%\newcommand\Monad		{{\mathbb M}}
%\newcommand\MS			{\mathbb M} % Multiset.
%\newcommand\MSIn			{\mathrel{\mbox{\small$\#$}}} % Multiset In.
%\newcommand\Nat			{{\mathbb N}}
%\newcommand\Natural		{\mathbb N}
%\newcommand\NNReal		{{\mathbb R}^\geq}
%\newcommand\nodet			{{s}}
%%\newcommand\nodet			{{y_-}}
%\newcommand\NoHeight[1]	{\raisebox{0pt}[0pt][0pt]{#1}}			
%\newcommand\Norm[1]		{\lfloor#1\rfloor} % Normalisation of a distribution.
%\newcommand\NotDemRef	{\mathrel{\not\Ref_\sqcap}}
%\newcommand\NotPrbRef		{\mathrel{\not\Ref_\#}}
%\newcommand\NotPRef		{\mathrel{\not\preccurlyeq}}
%\newcommand\NotRef		{\mathrel{\not\sqsubseteq}}
%\newcommand\NotRRef		{\mathrel{\not\sqsupseteq}}
%\newcommand\NotRefQ		{\mathrel{\not\sqsubseteq_{\mbox{\rm?}}}}
%\newcommand\NotRefQD		{\mathrel{\not\sqsubseteq'_{\mbox{\rm?}}}}
%\newcommand\NotRefQDD	{\mathrel{\not\sqsubseteq''_{\mbox{\rm?}}}}
%\newcommand\NotPRefQ		{\mathrel{\not\preceq_{\mbox{\rm?}}}}
%\newcommand\NotRefS		{\mathrel{\not\sqsubseteq_\circ}} % Structural refinement (not)
%\newcommand\NotRefT		{\mathrel{\not\sqsubseteq_{\GainFunc{}}}} % Testing refinement (not)
%\newcommand\NRefB		{\mathrel{\NotRef_\bot}}
%\newcommand\NRRefB		{\mathrel{\NotRRef_\bot}}
%\newcommand\NullChannel	{{\sf nc}}
%\newcommand\Obs			{\caly} % Used by Carroll for the Observation space. Change?
%\newcommand\OMin[1]		{\overline{#1}} % Abbreviation for "one minus", convenient in calculations.	
%\newcommand\OneC		{\mathds{1}} % Unit channel.
%\newcommand{\OneVect}		{\mathbf{1}} % all-ones vector
%\newcommand\OpenSem		{[\kern-.16em[}
%\newcommand\Output		{\mbox{$\cal O$}} % Channel output.
%\newcommand\Par			{\\~\\\quad} % For putting a paragraph break in an abstract.
%\newcommand\Parallel		{\mathbin{\parallel}} % For putting a paragraph break in an abstract.
%\newcommand\Part			{{\mathbb E}}
%\newcommand\PC[1]			{\PCI{#1}}
%\newcommand\PCE[1]		{\mathbin{{}_{#1}\kern-.05em\boxplus}}
%\newcommand\PCIp		{{\Cx\PCI{\textrm{\MPF{\textit p}}\kern-.1em}}} % 128364: With a meta-p. But just guesswork.
%\newcommand\PCEp		{{\Cx\PCE{\textrm{\MPF{\textit p}}\kern-.1em}}} % 128364.
%\newcommand\PCIP		{{\Cx\PCI{\textrm{\MPF{\textit P}\,}\kern-.1em}}} % 128364: With a meta-p. But just guesswork.
%\newcommand\PCEP		{{\Cx\PCE{\textrm{\MPF{\textit P}\,}\kern-.1em}}} % 128364.
%
%% I discovered 190222 that -many- program fragments were being combined with \oplus, which we recently
%% decided should be reserved for -internal- choice. Programs should be combined with external choice.
%% So I changed all the affected oplus's to obox's, but use the special macros below so that things could
%% be reversed if necessary.
%%\newcommand
%\newcommand\PCEwasPC[1]	{\PCE{#1}}
%\newcommand\PCIwasPC[1]	{\PCI{#1}}
%\newcommand\PCEFwasPCF	{\PCE{\NF{1}{2}}}
%\newcommand\PCIFwasPCF	{\PCI{\NF{1}{2}}}
%%\newcommand\MPC[1]		{\MPCI{#1}}
%\newcommand\MPC[1]		{\PCI{#1}} % For now, just use ordinary $p$.
%\newcommand\MPCI[1]		{\mathbin{{}_{\mbox{\tt\Meta{#1}}}\kern-.05em\oplus}}
%\newcommand\MPCE[1]		{\mathbin{{}_{\mbox{\tt\Meta{#1}}}\kern-.05em\boxplus}}
%\newcommand\PAR			{\mbox{$\interleave$}} % Concrete parallel, when distinction is necessary.
%\newcommand\PCIF			{\PCINF{1}{2}} % 0945: Abbreviation for fair choice.
%\newcommand\PCEF		{\PCENF{1}{2}} % 0945: Abbreviation for fair choice.
%\newcommand\PCINF[2]		{\PCI{\NF{#1}{#2}}} % 0944: Nicefrac built-in.
%\newcommand\PCENF[2]		{\PCE{\NF{#1}{#2}\,}} % 0944: Nicefrac built-in.
%\newcommand\MPF[1][\empty]	{\ifx\empty#1\empty\it\tt\else\mbox{\tt\Meta{#1}}\fi} % Program font: \PF sets it; \PF[x] applies it.
%\newcommand\PFor[1]		{{#1}_\ast} % Push forward.
%\newcommand\pGCL		{\textit{pGCL}}
%\newcommand\Point[1]		{[#1]} % Point distribution or hyper.
%%\newcommand\Pq			{:<~} % Probabilistic assignment in program texts.
%\newcommand\Pq			{:\kern-.2em$\in$~} % Probabilistic assignment in program texts.
%\newcommand\PrbRef		{\mathrel{\Ref_\#}}
%\newcommand{\PriorIn}[2]		{#1 \rangle #2}
%\newcommand\PRef			{\mathrel{\preccurlyeq}}
%\newcommand\PRefQ		{\mathrel{\preceq_{\mbox{\rm?}}}}
%\newcommand\QIF			{\textit{QIF}} % Quantitative Information Flow
%\newcommand\Rational		{\mathbb Q}
%\newcommand\RCf[1]		{\Rf{\Cx#1}}	% Carroll footnote for reviewer.
%\newcommand\Real			{\mathbb R} % Real numbers
%\newcommand\RealNN		{\Real_{\ge 0}} % Non-negative real numbers
%\newcommand\RefB			{\mathrel{\Ref_\bot}}
%\newcommand\RRefB		{\mathrel{\RRef_\bot}}
%\newcommand\RefQ			{\mathrel{\sqsubseteq_{\mbox{\rm?}}}}
%\newcommand\RefQD		{\mathrel{\sqsubseteq'_{\mbox{\rm?}}}}
%\newcommand\RefQDD		{\mathrel{\sqsubseteq''_{\mbox{\rm?}}}}
%\newcommand\RefS			{\mathrel{\sqsubseteq_\circ}} % Structural refinement
%\newcommand\RefT			{\mathrel{\sqsubseteq_{\GainFunc{}}}} % Testing refinement
%\newcommand\RESP		{resp.} % 1532.
%\newcommand\RMat[3]		{\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\hspace{#1}\left.\rule{0pt}{#3}\right)$}}}
%\newcommand\RRef			{\mathrel\sqsupseteq}
%\newcommand\RSA			{\textit{RSA}}
%\newcommand\Sem[1]		{\OpenSem#1\CloseSem}
%\newcommand\NRSeq		{\mathbb S} % Non-repeating sequence.
%\renewcommand\setminus		{-}
%\newcommand\SfA			{\textsf{A}} % 0847.
%\newcommand\SfB			{\textsf{B}} % 0847.
%\newcommand\SfC			{\textsf{C}} % 0847: Shortcut for channel matrix C.
%\newcommand\SfD			{\textsf{D}} % 0847.
%\newcommand\SfE			{\textsf{E}}
%\newcommand\SfJ			{\textsf{J}}
%\newcommand\Sfj			{\textsf{j}}
%\newcommand\SfS			{\textsf{S}}
%\newcommand\Sfs			{\textsf{s}}
%\newcommand\SfW			{\textsf{W}} % 0847.
%\newcommand\Size[1]		{|#1|} % Size (eg of a set).
%\newcommand\Skip			{\fbox{DEPRECATED}} % Deprecated.
%\newcommand\Sm[1]		{{\mbox{\small$#1$}}}
%\newcommand{\SmallSum}[1]{\textstyle{\sum_{#1}\:}}
%\newcommand\Span[1]			{\|#1\|} % span of function
%\newcommand\SP[1]			{[#1]} % Sub-point hyper.
%\newcommand\Spc[1]		{{\cal #1}} % Select font for input- or output space.
%\newcommand\Spot			{\mathbin{\mbox{\scriptsize$\bullet$}}} % 1144.
%\newcommand\SRef			{\mathrel{\sqsubset}}
%\newcommand\State			{\calx} % State space.
%\newcommand\StrictRef		{\mathrel\sqsubset}
%\newcommand\Strut[1][1]		{\rule{0pt}{#1ex}} % Make a strut.
%\newcommand\Subst[2]		{[{#1}$\backslash${#2}]}
%\newcommand\Sup			{\mathbin{\sqcup}} % Supremum, or binary maximum
%\newcommand\Tails			{\textit{tails}}
%\newcommand\Tau			{\textsf{T}}
%\newcommand\Th			{^{\textit{th}}}
%\newcommand\Then {\textbf{then}}
%\newcommand\To			{\textbf{to}} % 1159.
%\newcommand\Tr			{\textnormal{\textbf{tr}}}
%\newcommand\Trace[1]		{\Tr(#1)}	% trace of a matrix
%\newcommand\True			{\mbox{\it true}} % {\textit{true}}
%\newcommand\Ucl			{{\mathbb U}}
%\newcommand\UClose[1]		{#1^{\Union}}
%\newcommand\Unif			{{\sf uniform}}
%%\newcommand\Uniform		{\vartheta} % Looks like a curly "u". Alternatively \pi^u, but it a bit ``cluttery'' with its superscript, and in some places it was \sigma, and some \upsilon.
%\newcommand\Uniform		{{\mbox{\boldmath$\vartheta$}}} % Looks like a curly "u". Alternatively \pi^u, but it a bit ``cluttery'' with its superscript, and in some places it was \sigma, and some \upsilon.
%\newcommand\UniformSmall	{{\mbox{\scriptsize\boldmath$\vartheta$}}} % For use in super- and subscripts.
%
%\newcommand\UNION		{\mathop\cup}
%\newcommand\val			{\Spc{V}}	% Universe of values in statistical databases
%\newcommand\Val			{{\mathbb V}} % Valuations.
%\newcommand\valueitem		{\mathit{val}}	% values in statistical databases
%\newcommand\Var			{{\tt var}}
%\newcommand\Vb			{V}
%\newcommand\Vbmax		{V^\mathrm{max}}
%\newcommand\Vd			{V_\dx}
%\newcommand\VDist			{\overline{{\mathbb D}}}
%\newcommand\Vect[1]			{\mathbf{#1}}
%\newcommand\VHyp			{\overline{{\mathbb H}}}
%\newcommand\Vowel		{\textsf{Vowel}}
%\newcommand\Weight[1]		{\langle#1\rangle} % a partial distribution.
%\newcommand\WIDE[1] 		{~~~~~~#1~~~~~~} % Bigger space.
%\newcommand\WideDefs 		{~~\Defs~~~~~~~~} % More space on the right, for definitions.
%\newcommand\WLOG		{wlog.} % 1532: Don't forget \ afterwards.
%\newcommand\Wp			{{\sf wp}} % 0945.
%\newcommand\WPROB		{wprob.} % 1532.
%\newcommand\WRT			{wrt.} % 1532.
%\newcommand\WS[1]		{\mathbin{{}_{#1}\kern-.05em+}} % Weighted sum.
%\newcommand\WSNF[2]		{\WS{\nicefrac{#1}{#2}}} % 0944.
%\newcommand\WSF			{\WSNF{1}{2}} % 0945.
%\newcommand\wstar			{{w^{\star}}}
%\newcommand\XK			{\kern-.1em} % For horrible typesetting of \calx
%\newcommand\XS			{\texttt{xs}}
%\newcommand\XKK			{\kern-.2em}
%\newcommand\ZeroC		{\mathds{O}} % Zero channel.
%\newcommand{\ZeroVect}		{\mathbf{0}} % zero vector
%
%
%\newenvironment{ReCorollary}[2]	{\par\textit{Corollary \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}
%\newenvironment{ReLemma}[2]		{\par\textit{Lemma \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}
%\newenvironment{ReTheorem}[2]	{\par\textit{Theorem \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}
%\renewcommand\Join			{\mathrel{\sqcup}} % \Join defined in some package.
%
%%%% AKM has added these for the HMM section
%\newcommand\CM[2] {(#1{:}#2)}
%
%%%% AKM has added these for the Voting section
%\newcommand{\uniform}{\sigma}
%\newcommand{\PrivA}[1]{\alpha_{#1}}
%\newcommand{\PrivB}[1]{\#\alpha_{#1}}
%\newcommand{\PrivC}[1]{\neg \alpha_{#1}}
%\newcommand{\Hamming}[2]{\textbf{h}(#1,#2)}
%\newcommand{\RProd}{{\times}}
%
%%%% Mario has added these for axioms
%\newcommand{\qm}[1]{``#1''}
%%\newcommand{\nullchannel}{\ensuremath{\bar{0}}} % Use ZeroC
%%\newcommand{\idchannel}{\ensuremath{\bar{1}}} % Use OneC
%%\newcommand{\nonintchannel}{C\ensuremath{_{\textnormal{NI}}}}
%
%%%% Mario has added these for compositions
%\newcommand{\intchoice}[1]{\;{{}_{\mathit{#1}}{\oplus}}\;} % operator to be used among parameters: it gives nice spacing.
%\renewcommand\intchoice[1] {\PCI{{#1}}} % 181205: Temporary--- just trying it out.
%\newcommand{\intchoiceop}[1]{{}_{\mathit{#1}}{\oplus}} % name of the operator, to be used when no paramaters are needed.
%%\newcommand{\voper}{{}_{p}\cupdot}
%\newcommand{\extchoice}[1]{\;{{}_{\mathit{#1}}{\cupdot}}\;} % operator to be used among parameters: it gives nice spacing.
%\renewcommand\extchoice[1] {\PCE{{#1}}} % 181205: Temporary--- just trying it out.
%\newcommand{\extchoiceop}[1]{{}_{\mathit{#1}}{\cupdot}} % name of the operator, to be used when no paramaters are needed.
%\newcommand{\hyperc}[2]{[#1 \, \rangle \, #2]} % Hyper [\pi > C] created by pushing a prior \pi through a channel C
%\newcommand{\reals}{\mathbb{R}}
%\newcommand{\dist}{\mathbb{D}}
%\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\sqcup}}
%\newcommand{\ch}[2]{#1{\Fun}\Dist#2} % channel with input set #1 and output set #2
%\newcommand{\chset}[1]{{\Conc{C}_{#1}}} % set of all channels with input set #1
%
%\newcommand{\extcond}[1]{\;{{}_{\scriptscriptstyle #1}\triangle}\;} % external conditional operator to be used among parameters: it gives nice spacing.
%\renewcommand\extcond[1] {\mathbin{\triangleleft#1\triangleright}}
%\newcommand{\extcondop}[1]{{}_{\scriptscriptstyle #1}\triangle} % name of the external conditional operator, to be used when no paramaters are needed.
%\newcommand\triangleplus[1][2.07ex]{%
%	\renewcommand\stacktype{L}%
%	\mathbin{%
%		\scaleto{\stackon[0.9pt]{$\triangle$}{\tiny ${+}$}}{#1}%
%	}} % Used for contional operators.
%\newcommand{\intcond}[1]{\; {{}_{\scriptscriptstyle #1} \triangleplus }\;} % internal conditional operator to be used among parameters: it gives nice spacing.
%\renewcommand\intcond[1] {\mathbin{{\ll}#1{\gg}}}
%\newcommand{\intcondop}[1]{{}_{\scriptscriptstyle #1}\triangleplus} % name of the internal conditional operator, to be used when no paramaters are needed.
%
%\newcommand{\hchoice}[1]{\;{{}_{\mathit{#1}}{\oplus}}\;} % operator to be used among parameters: it gives nice spacing.
%\newcommand{\hchoiceop}[1]{{}_{\mathit{#1}}{\oplus}} % name of the operator, to be used when no paramaters are needed.
%\newcommand{\vchoice}[1]{\;{{}_{\mathit{#1}}{\cupdot}}\;} % operator to be used among parameters: it gives nice spacing.
%\newcommand{\vchoiceop}[1]{{}_{\mathit{#1}}{\cupdot}} % name of the operator, to be used when no paramaters are needed.
%\newcommand{\vifthen}[1]{\;{{}_{\scriptscriptstyle #1}\triangle}\;} % operator to be used among parameters: it gives nice spacing.
%\newcommand{\vifthenop}[1]{{}_{\scriptscriptstyle #1}\triangle} % name of the operator, to be used when no paramaters are needed.
%
%%%% Kostas has added these for the capacity section
%\newcommand\Kant[3]			{\KantA(#1)(#2,#3)} % Kantorovich distance
%\newcommand\KantA			{{\mathbb K}^{\!\scriptscriptstyle<}} % Kantorovich distance, no arguments
%\newcommand\KantK			{{\mathbb K}}
%\newcommand\Wass[3]			{{\mathbb W}(#1)(#2,#3)} % Wasserstein distance
%\newcommand\WassA			{{\mathbb W}} % Wasserstein distance, no arguments
%\newcommand\TotalVar		{\mathrm{tv}} % total variation distance
%\newcommand\DiscMetric		{\mathrm{dm}} % total variation distance
%\newcommand\AllOne			{{\mathbb O}} % So called because it's a right-zero for multiplication.
%\newcommand\LipDesc[2]				{$#1,#2$-Lipschitz}
%\newcommand\LipDescA[1]			{$#1$-Lipschitz}
%\newcommand\Lipschitz[3][\QuasiReal]	{{\mathbb C}^{#2,#1}{#3}} % Lipschitz set (contractions)
%\newcommand{\Extreme}		{\mathrm{ext}} % extreme points
%% \newcommand{\QuasiConvex}	{\Quasify{\GainOneSpanVg{}}}
%\newcommand{\QuasiConvex}	{\mathbf{q}}
%\newcommand{\QuasiReal}		{\Quasify{\Real}}
%\newcommand{\QuasiRealN}	{\Quasify{\Real^n}}
%\newcommand{\QuasiGain}		{\Quasify{\calg}}
%\newcommand{\QuasiGainOne}	{\Quasify{\GainOneSpan{}}}
%\newcommand{\Quasify}[1]	{{	% quasimetric d^< symbol, with #1 as subscript.
%	\mathchoice					% use \mathchoice for better scaling
%		{d_{#1}^{\scalebox{.6}{$<$}}} 						% displaystyle
%		{d_{#1}^{\scalebox{.6}{$<$}}} 						% textstyle
%		{d_{#1}^{\scalebox{.4}{$<$}}} 						% scriptstyle
%		{d_{\scalebox{.45}{$#1$}}^{\scalebox{.45}{$<$}}}	% scriptscriptstype
%}}
%\newcommand{\UpDownStr}		{\stretchrel*{\updownarrow}{\dag}}	% symbol for 1-spanning Vg's, same height as a \dag
%
%%%% Mario has added these for Priors as Hypers
%\usepackage{cancel} % Allows for \cancel
%\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\argmin}{argmin}
%%\DeclareMathOperator*{\E}{\mathlarger{\mathlarger{\mathbb{E}}}}
%%% Macros for this chapter here. Integrate them into the main MacrosMaths later.
%\newcommand{\distv}{\mathbb{V}}
%\newcommand{\hyperv}{\widehat{\mathbb{V}}}
%
%\newcommand{\interior}{\mathrm{int}}
%\newcommand{\boundary}{\mathrm{bd}}
%\newcommand{\bbd}{\mathbb{D}}
%\newcommand{\epi}{\mathrm{epi}}
%
%\newcommand\WSum[1]{\mathbin{_{#1}+}}
%%\newcommand\DELTA {\underline{\Delta}}
%
%\newcommand\DPI {\textit{DPI}}
%\newcommand{\dpi}{\texttt{DPI}}
%%\newcommand{\nonneg}{\texttt{MONO}} 
%\newcommand{\mono}{\texttt{MONO}} 
%\newcommand{\nonint}{\texttt{NI}} 
%\newcommand{\cvx}{\texttt{CVX}}
%\newcommand{\quasicvx}{\texttt{Q-CVX}}
%\newcommand{\avg}{\texttt{AVG}}
%\newcommand{\ubound}{\texttt{UBND}}
%\newcommand{\lbound}{\texttt{LBND}}
%\newcommand{\bounds}{\texttt{BNDS}}
%\newcommand{\cnty}{\texttt{CNTY}}
%\newcommand{\worst}{\texttt{MAX}}
%\newcommand{\RelInt}[1]{\textnormal{relint}(#1)}
%% \newcommand{\Transp}{\texttt{TRSP}}
%
%%%% Macros extracted (in haste) from the non-termination chapter 180524.
%% Rationalise them later, and put them in place above.
%\newcommand\CalX		{\calx}
%\newcommand\CalY		{\caly}
%\newcommand\Chap[1]	{\Chp{#1}}
%\newcommand\SubDist	{\underline{\Dist}}
%\newcommand{\TRef}	{\leq}
%\newcommand{\PSecRef}	{\preceq}
%
%
%
%
%%%% These are macros we've used in our papers, but have not yet used here in the book.
%%%% I moved them down here to make the list above less cluttered.
%%%% If there's one here you like/need, just move it back.
%
%%\newcommand\Atimes		{\times} % Arithmetic multipication of scalars,
%%\newcommand\basicgain[1]	{\cal{E}#1}
%%\newcommand\calc		{\mathcal{C}}	% Contexts
%%\newcommand\cals		{\Spc{S}}
%%\newcommand\calu		{\Spc{U}}
%%\newcommand\CDist[1]		{|\!| #1 |\!|_C}
%%\newcommand\ChPar[2]		{#1{\parallel}#2}
%%\newcommand\Col[2]		{#1_{-,#2}} % Dash for "all rows".
%%\newcommand\DistEnum[1]	{\{\kern-.2em\{#1\}\kern-.2em\}}
%%\newcommand\End 		{\hfill$\Box$}
%%\newcommand\finitegain[1]	{\cal{G}#1}
%%\newcommand\GAdd[2]		{#1_{+#2}}
%%\newcommand\GAddX[3]	{#1_{+#2@#3}} 
%%\newcommand\GMult[2]		{#1_{\times#2}}
%%\newcommand\GVul[2]		{V_{#2}{#1}} % Backwards because the g-test is a postcondition.
%%\newcommand\Iff			{\Leftrightarrow}
%%\newcommand\Imp			{\Rightarrow}
%%\newcommand\IS[3]		{#1[#2=+#3]}
%%\newcommand\KantDist[1]	{|\!| #1 |\!|_K}
%%\newcommand\KDist[3]		{{\mathbb K}_{#3}(#1,#2)} % Kantorovich distance
%%\newcommand\Ker			{\mathop{\rm ker}}
%%\newcommand\LiftBox		{\vspace{-1em}} % Avoid extra space when display ends environment.
%%\newcommand\LMat[3]		{\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\left(\rule{0pt}{#3}\right.\hspace{#1}$}}}
%%\newcommand\MCapty[3]	{\mathcal{L}_{#2}(#3,#1)}
%%\newcommand\Nrm		{{\sf nrm}}
%%\newcommand\Num[1]		{#1^{\textrm{\scriptsize\#}}}
%%\newcommand\RevealAll[1]	{\textit{RevealAll}(#1)}
%%\newcommand\RMat[3]		{\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\hspace{#1}\left.\rule{0pt}{#3}\right)$}}}
%%\newcommand\Row[2]		{#1_{#2,-}} % Dash for "all columns".
%%\newcommand\Smallsum[1]	{\textstyle{\sum_{#1}\:}} % Another less aggressive version.
%%\newcommand\Spot		{\mathbin{\mathbold{\cdot}}} % 1144:The mathbold doesn't seem to work.
%%\newcommand\Sum[1]		{\Sigma#1} % Less aggressive symbol than \sum.
%%\newcommand\WDist[3]		{{\mathbb W}_{#3}(#1,#2)} % Wasserstein distance
%%\newcommand\WIDE[1]		{\Wide{\Wide{#1}}} % Extra wide space.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% GET \smalltriangleright from mathabx without loading it (conflicts with newtxmath)
%% Setup the mathb font (from mathabx.sty)
%\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
%\DeclareFontShape{U}{mathb}{m}{n}{
%      <5> <6> <7> <8> <9> <10> gen * mathb
%      <10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
%      }{}
%\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
%% Define a subset character from that font (from mathabx.dcl)
%\DeclareMathSymbol{\smalltriangleright}{2}{mathb}{"9B}% name to be checked
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%
%
%
%
%
%%--- \newcommand\bft{\mathsf{bft}}
%%--- \newcommand{\ct}{\mathsf{ct}}
%%--- \newcommand{\Et}{\mathsf{bv}}
%%--- \newcommand{\Etv}{\mathsf{brv}}
%%--- \newcommand{\Etp}{\mathsf{brp}}
%%--- \newcommand{\Ft}{\mathsf{flt}}
%%--- \newcommand{\Ht}{\mathsf{H}}
%%--- \newcommand\CCL {\mathsf{ccl}} % convex closure
%%--- \newcommand\app{\mathsf{app}}
%%--- \newcommand{\Apply}{\mathsf{app}}
%%--- \newcommand\Vh {\mathsf{h}}
%%--- \newcommand\Vv {\mathsf{v}}
%%--- \newcommand\Va {\mathsf{a}}
%%--- \providecommand\Vb {\mathsf{b}}
%%--- \newcommand\Vc {\mathsf{c}}
%%--- \providecommand\Vd {\mathsf{d}}
%%--- \newcommand\Vj {\mathsf{j}}
%%--- \newcommand\Vx {\mathsf{x}}
%%--- \newcommand\Vy {\mathsf{y}}
%%--- \newcommand\Vm {\mathsf{m}}
%%--- \newcommand\Vn {\mathsf{n}}
%%--- \newcommand\BftMin{\mathbin{\oslash}}
%%--- \newcommand{\Peq}{\equiv}
%%--- \newcommand{\Pge}{\mathrel\LLeftarrow}
%%--- \newcommand{\Ple}{\mathrel\RRightarrow}
%%--- \newcommand\st {\mathrel{\Spot}}
%%--- \newcommand\VV {{\cal V}}
%%--- \newcommand\NLg {\textrm{l}\overline{\textrm{g}}}
%%--- \renewcommand\NLg {\overline{\lg}}
%%--- \newcommand\DD {{\cal D}}
%%--- \newcommand\SeqCC[1] {(-\,;\,#1)}
%%--- \newcommand\HH {{\cal H}}
%%--- \newcommand\Atomic[1] {\AtomicOpen#1\AtomicClose}
%%--- \newcommand\AtomicOpen {\langle\!\langle}
%%--- \newcommand\AtomicClose {\rangle\!\rangle}
%%--- \newcommand\Rel {\mathbin{\leftrightarrow}}
%%--- \newcommand\Dom {\mathsf{dom}}
%%--- \newcommand\Ran {\mathsf{ran}}
%%--- \newcommand\NPow {\mathsf P}
%%--- \newcommand\TDist {\mathsf{D}}
%%--- \newcommand\Uniform[1] {\PSet{}{}{#1}}
%%--- \newcommand\Support[1] {{\lceil #1 \rceil}}
%%--- \newcommand{\Transpose}[1]{{#1}^{\mathbf{T}}} % transpose of a matrix
%%--- \newcommand\Above {\mathbin{\raisebox{-.15em}{+}\kern-.39em\raisebox{.15em}{\makebox[0pt]{$+$}}\kern.45em}}
%%--- \newcommand\AboveRel {~\mathrel{\Above}~}
%%--- \newcommand\Beside {{+}\kern-.5em{+}}
%%--- \newcommand\BesideRel {\mathrel{\Beside}}
%%--- \newcommand\IdM[1] {{\mathsf 1}_{#1}}
%%--- \newcommand\DiagM[1] {\backslash\kern-.35em\backslash\kern-.05em\mbox{\small$#1$}\kern-.05em\backslash\kern-.35em\backslash}
%%--- \newcommand{\ISeq}{{\mathsf{iseq}}}
%%--- \newcommand\BF {Big Fat}
%%--- \newcommand\GGA {\textsf{gg}}
%%--- \newcommand\MaxW {\mathbin{\textbf{max}}}
%%--- \newcommand\MAX {\sqcup}
%\newcommand\MIN {\sqcap}
%%--- \newcommand\UMax[1] {{\def\Cond{#1}\ifx\Cond\empty {\sqcup} \else {\sqcup}^{#1} \fi}}
%%--- \newcommand\UMin[1] {{\def\Cond{#1}\ifx\Cond\empty {\sqcup} \else {\sqcap}^{#1} \fi}}
%%--- \newcommand\Max[1] {\MAX_{#1}}
%%--- \newcommand\List[1] {\langle#1\rangle}
%%--- \newcommand\Finer {\mathrel{\raisebox{0.2ex}{$\sqsubset$}\kern-.8em\raisebox{-1.1ex}{$\sim$}}}
%%--- \newcommand\StrictFiner {\mathrel{\raisebox{0.2ex}{$\sqsubset$}\kern-.8em\raisebox{-1.1ex}{${\sim}\kern-.55em\raisebox{.15em}{\tiny$/$}$}\kern.4em}}
%%--- \newcommand\Coarser {\mathrel{\raisebox{0.2ex}{$\sqsupset$}\kern-.8em\raisebox{-1.1ex}{$\sim$}}}
%%--- \newcommand\SimFiner {\mathrel{\approx}}
%%--- \newcommand\Similar {\mathrel{\approx}}
%%--- \newcommand\NotSimilar {\mathrel{\not\approx}}
%%--- \newcommand\EquivRef {\mathrel{\equiv}}
%%--- \newcommand\ORef[1] {\mathrel{\preceq_{#1}}}
%%--- \newcommand\StrictORef[1] {\mathrel{\prec_{#1}}}
%%--- \newcommand\ORefB[1] {\mathrel{\succeq_{#1}}}
%%--- \newcommand\NotORef[1] {\mathrel{\not\preceq_{#1}}}
%%--- \newcommand\ERef {\mathrel{\preceq}}
%%--- \newcommand\ERefB {\mathrel{\succeq}}
%%--- \newcommand\NotERef {\mathrel{\not\preceq}}
%%--- \newcommand\BRef {\mathrel{\preceq_\Bt}}
%%--- \newcommand\NotBRef {\mathrel{\not\preceq_\Bt}}
%%--- \newcommand\StrictBRef {\mathrel{\prec_\Bt}}
%%--- \newcommand\HRef {\mathrel{\preceq_\Ht}}
%%--- \newcommand\NotHRef {\mathrel{\not\preceq_\Ht}}
%%--- \newcommand\StrictHRef {\mathrel{\prec_\Ht}}
%%--- \newcommand\GRef[1] {\mathrel{\preceq_{\Gt{#1}}}}
%%--- \newcommand\NotGRef[1] {\mathrel{\not\preceq_{\Gt{#1}}}}
%%--- \newcommand\ARef {\sqsupseteq}
%%--- \newcommand{\RefMatrices}{{\cal R}}
%%--- \newcommand{\FinerMatrices}{{\cal M}} % for siMple
%%--- \newcommand{\StratMatrices}{{\cal G}}
%%--- \newcommand{\GStratMatrices}{{\cal K}} % running out of letters...
%%--- \newcommand{\UnitMatrix}{{\bf 1}}
%%--- \newcommand{\ZeroMatrix}{{\bf 0}}
%%--- \newcommand{\DRef}{\Ref_{\Dist{}}} % distribution order
%%--- \newcommand{\QDRef}{\Ref_{R}}      % quantum distribution order
%%--- \newcommand{\NotQDRef}{\mathrel{\not{\QDRef}}}
%%--- \newcommand{\TQDRef}{\Ref_{T}}      % quantum distribution testing order
%%--- \newcommand{\NotTQDRef}{\mathrel{\not{\TQDRef}}}
%%--- \newcommand{\EDRef}{\Ref_{ET}}
%%--- \newcommand{\NotEDRef}{\mathrel{\not{\EDRef}}}
%%--- \newcommand{\FDRef}{\Ref_{FT}}
%%--- \newcommand{\NotFDRef}{\mathrel{\not{\FDRef}}}
%%--- \newcommand{\FRef}{\Ref_{FT}}
%%--- \newcommand{\NotFRef}{\mathrel{\not{\FRef}}}
%%--- \newcommand{\CRef}{\Ref_{C}}
%%--- \newcommand{\NotCRef}{\mathrel{\not{\FRef}}}
%%--- \newcommand{\SSRef}{\Ref_{S}}      % Shadow set distribution order
%%--- \newcommand{\Fracs}{\textsf{fracs}}    % Note: moved from document
%%--- \newcommand\NGets {{:}{\in}\,}
%%--- \newcommand\PGets {{\NGets}}
%%--- \newcommand\If {\textbf{if}}
%%--- \newcommand\Then {\textbf{then}}
%%--- \newcommand\Else {\textbf{else}}
%%--- \newcommand\Elseif {\textbf{else if}}
%%--- \newcommand\Fi {\textbf{fi}}
%%--- \newcommand\Reveal {\Leak}
%%--- \newcommand\Vpk {v'\kern-.25em}
%%--- \newcommand\MatSem[2][*] {\def\z{#1}\if*\z (\!(#2)\!) \else \left(\kern-.3em\left(\rule{0pt}{#1}#2\right)\kern-.3em\right) \fi}
%%--- \newcommand\MatSemC[1] {(\kern-.21em\raisebox{.025em}{\small$\mid$}#1\raisebox{.025em}{\small$\mid$}\kern-.22em)}
%%--- \newcommand\SemC[1] {[\![#1]\!]_C}
%%--- \newcommand\Or {\mathbin{\sqcap}}
%%--- \newcommand\UC[1] {\mathbin{_{#1}\uplus}} % prob. unification between multisets
%%--- \newcommand\TT {\textsf{T}}
%\newcommand\Xor {\mathbin{\nabla}}
%%--- \newcommand\Spec[2]{#1{:}[#2]}
%%--- \newcommand\Vis {\textbf{vis}}
%%--- \newcommand\Hid {\textbf{hid}}
%%--- \newcommand\While {\textbf{while}}
%%--- \newcommand\Do {\textbf{do}}
%%--- \newcommand\Od {\textbf{od}}
%%--- \newcommand{\ABegin}{\langle \!\langle}
%%--- \newcommand{\AEnd}{\rangle \! \range}
%%--- \newcommand{\Quantum}[1]{\QBegin #1 \QEnd} % Quantum program semantics of #1
%%--- \newcommand{\Prob}[1]{\QBegin #1 \QEnd} % Probabilistic program semantics of #1
%%--- \newcommand{\Shadow}[1]{\QBegin #1 \QEnd} % Shadow program semantics of #1
%%--- \newcommand{\Std}[1]{\QBegin #1 \QEnd} % Standard program semantics of #1
%%--- \newcommand{\QBegin}{{ [\!\!\mid }}
%%--- \newcommand{\QEnd}{{ \mid\!\!] }}
%%--- \newcommand{\LeftPS}{ \{\!\!\{ }
%%--- \newcommand{\RightPS}{ \}\!\!\} }
%%--- \newcommand{\AddShadow}{\mathsf{atomic}} % was embed
%%--- \newcommand{\Hide}{\mathsf{embed}} % was hide
%%--- \newcommand\InQuadL[1] {\makebox[0pt][l]{$#1$}\quad}
%%--- \newcommand\InQuadR[1] {\quad\makebox[0pt][r]{$#1$}}
%%--- \newcommand\IF {\textbf{if}}
%%--- \newcommand\Flr[2]{{\lfloor #1 \rfloor_{#2}}}
%%--- \newcommand\Ceil[2]{{\lceil #1 \rceil_{#2}}}
%%--- \newcommand\Rnd[2]{[#1]_{#2}}
%%--- \newcommand\Module {\textbf{module}}
%%--- \newcommand\Int {\textbf{int}}
%%--- \newcommand\Public {\textbf{public}}
%%--- \newcommand\Private {\textbf{private}}
%%--- \newcommand\Init {\textbf{init}}
%%--- \newcommand\Return {\textbf{return}}
%%--- \newcommand\PP {{{+}{+}}}
%%--- \newcommand\MM {{-}{-}}
%%--- \newcommand\Pp[1] {[#1]}
%%--- \newcommand\TBC {\medskip\noindent\dotfill~To be continued~\dotfill}
%%--- \newcommand\ELSE {\textbf{else}}
%%--- \newcommand\Comment[1] {\makebox[0pt][l]{\quad\textrm{\small$\Leftarrow$~#1}}}
%%--- \newcommand\POINT {\textsf{U}}
%%--- \newcommand\LIFT {\textsf{L}}
%%--- \newcommand\SQUASH {\textsf{Q}}
%%--- \newcommand\MAP {\textsf{M}}
%%--- \newcommand{\HIDE}{\textsf{E}} % Now defined to be E for "embed" as in \Hide 
%%--- \newcommand{\PART}{\textsf{P}}
%%--- \newcommand{\OutV}{\textsf{outV}}
%%--- \newcommand\IIFrac[2] {\mbox{$\frac{#1}{#2}$}} % Frac in inline mode, slightly smaller.
%%--- \newcommand\IFrac[2] {\mbox{\small$#1/#2$}} % Frac in inline mode, slightly smaller.
%%--- \newcommand\SumSmall {\mbox{$\sum$}}
%%--- \newcommand\DSum {\mathop{\sum\kern-1em\sum}}
%%--- \newcommand\DSUM {\mathop{\sum\kern0em\sum}}
%%--- \newcommand{\EXP}{\mathop{\sum\kern-.45cm\sum}}
%%--- \renewcommand{\EXP}{+}
%%--- \renewcommand{\EXP}{{\cal E}}
%%--- \renewcommand{\EXP}{\otimes}
%%--- \renewcommand{\EXP}{\odot}
%%--- \renewcommand{\EXP}{{\cal E}\kern-.2em}
%%--- \newcommand\Exp[2]{(\kern-.25ex\EXP\,#1\bgroup\def\Elem{#2}\ifx\Elem\empty\egroup\else\egroup\mathrel{\Spot}#2\fi)}
%%--- \newcommand\ExpNorm[2]{[\kern-.1ex\EXP\,#1\bgroup\def\Elem{#2}\ifx\Elem\empty\egroup\else\egroup\mathrel{\Spot}#2\fi]}
%%--- \newenvironment{TJFigure}[2][t]{\begin{figure}[#1]\def\Label{#2}\small}{\label{\Label}\end{figure}}
%%%% MacrosGeneral 11 April 2017. 
%
%% Load a package only if the needed command is undefined. Makes usepackage self-documented,
%% plus it avoids loading unnecessary packages if the command is already defined elsewhere.
%\providecommand{\UsePackageFor}[2]{ \ifx#2\undefined\usepackage{#1}\fi }
%
%%%% Our packages
%%	If you add (or uncomment) a package, please include a comment to say
%%	who you are and what's using the package. (They're in alphabetical order.)
%%
%%   I've cleaned up the list, merging packages from main.tex (eg Three Judges),
%%   except those from Springer that went to StyleSvmono.tex.
%%
%% Nice one Kostas!
%\usepackage{silence}						% for supressing useless warnings
%	\WarningFilter{latex}{Marginpar on page}		% \thepage\space moved}
%	\WarningFilter{latex}{LaTeX Font Warning} 
%	\WarningFilter{latex}{Package hyperref Warning}
%	\WarningFilter{latex}{LaTeX Warning: Citation}
%	\WarningFilter{latex}{Overfull \hbox}
%	\WarningFilter{latex}{Underfull \hbox}
%
%\UsePackageFor{amsfonts}		{\mathbb}
%\UsePackageFor{amsmath}		{\text}
%\UsePackageFor{amssymb}		{\preccurlyeq}
%\usepackage{bbding}				% For the small pencil.
%\usepackage{blkarray}			% blockarray environment
%
%\usepackage{polytable}			% blkarray needs this for multicolumn: don't know why
%\let\True\undefined\let\False\undefined\let\Or\undefined % Uggh: These definitions "escape" from polytable.
%
%% Disabled temporarily CCM 180725
%\usepackage{chapterbib}			% For per-chapter references
%
%\usepackage{dsfont}				% For double-stroke numbers (eg 1 and 0 as identity and zero).
%\usepackage{endnotes}			% For endnotes.
%\usepackage{enumerate}			% For custom enumerations.
%\usepackage{graphicx}			% Including pictures etc.
%\usepackage{hyperref}			% for hyperlinks, configured later with \hypersetup
%\usepackage{latexsym}
%\usepackage{listings}			% 0923: For programs and ASCII: see environments for that.
%\usepackage{longtable}			% For tables that go over pages.
%\usepackage{makeidx}			% for index generation
%\usepackage{pdfpages}			% For including pdf files in the output.
%\UsePackageFor{scalerel}		{\stretchrel}
%\usepackage{stackengine}		% To allow for \stackanchor
%\usepackage{stmaryrd}			% For the parallels.
%\UsePackageFor{subfigure}	{\subfigure}	% Small figures combined into one (older/obsolete package); incompatible with subcaption.
%\usepackage{tikz}				% For drawings
%\usepackage[normalem]{ulem}		% For strikethroughs.
%\usepackage{units}				% For \nicefrac.
%\usepackage{url}				% For allowing urls.
%\usepackage{verbatim}			% For enviroment {comment}
%\usepackage{version}			% For version control (wrt eg to Answers}
%\usepackage{wasysym}			% For \smiley and \hexagon.
%\usepackage{wrapfig}
%\usepackage{xcolor}				% For colours.
%\usepackage{xspace}				% To {\Skip} space between command and argument
%
%% Used in the past, might be needed in the future
%%
%%\usepackage{amscd}
%%\usepackage{eufrak}			% For Fraktur (ueber-hypers); not needed if amsfonts alreaady loaded.
%%\usepackage{mathrsfs}
%%\usepackage{subcaption}		% Several figures combined (newer package); incompatible with subfigure and subfig.
%%\usepackage{txfonts}			% For the (temporary) refinement symbol. !CAREFUL! this changes all math fonts, there are ways to extract just one symbol!
%
%
%% hyperlinks (eg \ref's) should be colored blue. % 200125: Now coloured black.
%% Use {\hypersetup{hidelinks} ... } to disable them locally (eg in the TOC)
%\hypersetup{
%%	colorlinks=false, % 200119: Maybe this is a more reliable link-colour suppresser. No --- then it puts little boxes.
%	colorlinks=true,
%%	linkcolor=blue, 
%	linkcolor=black,  	% For Carroll, from Catuscia: uncomment this line and comment the previous one to eliminate the coloring of the hyperlinks.
%	urlcolor=black
%}
%
%% Ignore if file does not exist, as \include does, but use \input so that we're not  affected by \includeonly.
%\newcommand\InputIfExists[1]{\IfFileExists{#1}{\input{#1}}{}}
%
%%%% Assorted extras
%
%% http://tex.stackexchange.com/questions/32597/vertically-centered-horizontal-rule-filling-the-rest-of-a-line
%\def\Vhrulefill{\leavevmode\leaders\hrule height 0.7ex depth \dimexpr0.4pt-0.7ex\hfill\kern0pt}
%
%
%%%% Graphic helper
%%
%
%% \ImageInText{upNudge}{rightNudge}{scaleFactor}{fileName}
%\newcommand\ImageInText[4]%
%{\makebox[0pt][l]{%
%{\def\Up{#1}\def\Right{#2}% Use \def in case they're already defined.
%\hfill%
%\raisebox{\Up}[0pt][0pt]{% No height, no depth.
%\makebox[0pt][l]{\hspace{\Right}% No width.
%\includegraphics[scale=#3]{#4}%
%}}}}}
%
%% \ImageInTextBlock{height}{depth}{width}{upNudge}{rightNudge}{scaleFactor}{fileName}
%\newcommand\ImageInTextBlock[7]%
%{\def\Height{#1}% Use \def in case they're already defined.
%\def\Depth{#2}
%\def\Width{#3}
%\def\Up{#4}
%\def\Right{#5}
%\raisebox{\Up}[\Height][\Depth]{\makebox[\Width][l]{\hspace{\Right}\includegraphics[scale=#6]{#7}
%}}\\} % Without the \\ the following line is not separated by \Depth.
%
%%%% Make temporary (no parameter) command.
%\newcommand\TempCommand[2]{\providecommand#1{}\renewcommand#1{#2}}
%
%%%% Theorems, figures, footnotes etc.
%%
%
%% These already defined by Springer.
%%\newtheorem{theorem}{Theorem}
%%\newtheorem{corollary}[theorem]{Corollary}
%%\newtheorem{definition}[theorem]{Definition}
%%\newtheorem{lemma}[theorem]{Lemma}
%%\newtheorem{exercise}[theorem]{Exercise}
%
%% Uppercase theorems ended up being seldom used; most places in all parts of the book
%% use the standard environments. So I made them synonyms, we need a consistent style across
%% the book. We can easily customize the standard environments anyway if we want.
%% Kostas 180506
%
%% Uppercase theorems etc are now used everywhere. CCM 190803.
%
%\newcommand\FirstLineOfTheorem[1][\empty]{#1}
%\newcommand\MakeFact[2]{\newenvironment{#1}[2]{\begin{#2}[##1]\label{##2}\FirstLineOfTheorem}{\end{#2}}}
%
%% \newcommand\FirstLineOfTheorem[1][\empty] {\ifx#1\empty\quad\else~\hrulefill~#1\\\fi}
%% \newcommand\MakeFact[2]{\newenvironment{#1}[2]{\begin{#2}\label{##2}\textit{##1}\rm\noexpand\noexpand\FirstLineOfTheorem}{\hfill$\Box$\end{#2}}}
%%\newcommand\MakeFactGrey[2]{\newenvironment{#1}[2]{\begin{#2}\label{##2}\begin{svgraybox}\textit{##1}\rm\noexpand\noexpand\FirstLineOfTheorem}{\hfill$\Box$\end{svgraybox}\end{#2}}} % Gets "floats lost".
%
%%\MakeFact{Definition}{definition}
%%\MakeFact{Corollary}{corollary}
%%\MakeFact{Lemma}{lemma}
%%\MakeFact{Theorem}{theorem}
%%\MakeFact{Example}{example}
%%\MakeFact{Exercise}{exercise}
%
%% Hack to avoid double \qed's: \begin{Theorem} turns it on; and \begin{Proof} turns it off. \end{Theorem} adds a \qed only if it's off, and then turns it off unconditionally.
%\newif\ifNeedQED
%
%\newenvironment{Figure}[1][]{\ifx&#1&\begin{figure}\else\begin{figure}[#1]\fi}{\end{figure}}
%% SLightly tricky to put the glossary-capture within the Figure environment, because
%% the \label has to come after the \caption.
%\newcommand\FigLabel[1]{\label{#1}\glossary{Figure \ref{#1}}}
%
%\newenvironment{Definition}[1][]{% Deprecated.
%	\ifx&#1&\begin{definition}\else\begin{definition}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\qed\end{definition}}
%
%\newenvironment{DefinitionL}[2][]{
%	\ifx&#1&\begin{definition}\else\begin{definition}[#1]\fi
%	\label{#2}
%	\glossary{Definition \ref{#2}}
%	}{\qed\end{definition}}
%
%\newenvironment{ConjectureL}[2][]{
%	\ifx&#1&\begin{conjecture}\else\begin{conjecture}[#1]\fi
%	\label{#2}
%	\glossary{Conjecture \ref{#2}}
%	}{\qed\end{conjecture}}
%
%\newenvironment{ProblemL}[2][]{
%	\ifx&#1&\begin{problem}\else\begin{problem}[#1]\fi
%	\label{#2}
%	\glossary{Problem \ref{#2}}
%	}{\qed\end{problem}}
%
%\newenvironment{AlgorithmL}[2][]{
%	\ifx&#1&\begin{algorithm}\else\begin{algorithm}[#1]\fi
%	\label{#2}
%	\glossary{Algorithm \ref{#2}}
%	}{\qed\end{algorithm}}
%
%\newenvironment{Corollary}[1][]{% Deprecated
%	\global\NeedQEDtrue\ifx&#1&\begin{corollary}\else\begin{corollary}[#1]\fi}
%	{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{corollary}}
%
%\newenvironment{CorollaryL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{corollary}\else\begin{corollary}[#1]\fi
%		\label{#2}
%		\glossary{Corollary \ref{#2}}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{corollary}}	
%
%\newenvironment{Lemma}[1][]{% Deprecated.
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{lemma}\else\begin{lemma}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{lemma}}
%
%\newenvironment{LemmaL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{lemma}\else\begin{lemma}[#1]\fi
%		\label{#2}
%		\glossary{Lemma \ref{#2}}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{lemma}}
%
%\newenvironment{Proposition}[1][]{% Deprecated
%	\global\NeedQEDtrue\ifx&#1&\begin{proposition}\else\begin{proposition}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{proposition}}
%
%\newenvironment{PropositionL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{proposition}\else\begin{proposition}[#1]\fi
%		\label{#2}
%		\glossary{Proposition \ref{#2}}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{proposition}}
%
%\newenvironment{Example}[1][]{% Deprecated.
%	\ifx&#1&\begin{example}\else\begin{example}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\qed\end{example}}
%
%\newenvironment{ExampleL}[2][]{
%	\ifx&#1&\begin{example}\else\begin{example}[#1]\fi
%	\label{#2}
%	\glossary{Example \ref{#2}}
%	}{\qed\end{example}}
%
%\newenvironment{Exercise}[1][]{
%	\ifx&#1&\begin{exercise}\else\begin{exercise}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\qed\end{exercise}}
%
%\newenvironment{ExerciseL}[2][]{
%	\ifx&#1&\begin{exercise}\else\begin{exercise}[#1]\fi
%	\label{#2}
%	\glossary{Exercise \ref{#2}}
%	}{\qed\end{exercise}}
%
%\newenvironment{Theorem}[1][]{% Deprecated
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{theorem}\else\begin{theorem}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{theorem}}
%
%\newenvironment{TheoremL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{theorem}\else\begin{theorem}[#1]\fi
%		\label{#2}
%		\glossary{Theorem \ref{#2}}
%	}{\ifNeedQED\qed\else\relax\fi\global\NeedQEDfalse\end{theorem}}
%
%\newenvironment{Proof}{\global\NeedQEDfalse\begin{proof}}{\qed\end{proof}}
%
%%Trying out the hypothesis that grey items don't need an end-symbol.
%\newenvironment{GrayDefinition}[1][]{% Deprecated.
%	\ifx&#1&\begin{graydefinition}\else\begin{graydefinition}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{graydefinition}}
%
%\newenvironment{GrayDefinitionL}[2][]{
%	\ifx&#1&\begin{graydefinition}\else\begin{graydefinition}[#1]\fi
%	\label{#2}
%	\glossary{\textbf{Definition \ref{#2}}}
%	}{\end{graydefinition}}
%
%\newenvironment{GrayDefinitionLP}[2][]{ % Experimental same-page version.
%	\begin{samepage}
%	\ifx&#1&\begin{graydefinition}\else\begin{graydefinition}[#1]\fi
%	\label{#2}
%	\glossary{\textbf{Definition \ref{#2}}}
%	\samepage
%	}{\end{graydefinition}\end{samepage}}
%
%\newenvironment{GrayConjectureL}[2][]{
%	\ifx&#1&\begin{grayconjecture}\else\begin{grayconjecture}[#1]\fi
%	\label{#2}
%	\glossary{\textbf{Conjecture \ref{#2}}}
%	}{\end{grayconjecture}}
%
%\newenvironment{GrayCorollary}[1][]{% Deprecated.
%	\ifx&#1&\begin{graycorollary}\else\begin{graycorollary}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{graycorollary}}
%
%\newenvironment{GrayCorollaryL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{graycorollary}\else\begin{graycorollary}[#1]\fi
%		\label{#2}
%		\glossary{\textbf{Corollary \ref{#2}}}
%	}{\ifNeedQED\relax\else\relax\fi\global\NeedQEDfalse\end{graycorollary}}	
%
%\newenvironment{GrayLemma}[1][]{% Deprecated.
%	\ifx&#1&\begin{graylemma}\else\begin{graylemma}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{graylemma}}
%
%\newenvironment{GrayLemmaL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{graylemma}\else\begin{graylemma}[#1]\fi
%		\label{#2}
%		\glossary{\texbf{Lemma \ref{#2}}}
%	}{\ifNeedQED\relax\else\relax\fi\global\NeedQEDfalse\end{lemma}
%}
%
%\newenvironment{GrayExample}[1][]{% Deprecated.
%	\ifx&#1&\begin{grayexample}\else\begin{grayexample}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{grayexample}}
%
%\newenvironment{GrayExampleL}[2][]{
%	\ifx&#1&\begin{grayexample}\else\begin{grayexample}[#1]\fi
%	\label{#2}
%	\glossary{\textbf{Example \ref{#2}}}
%	}{\end{grayexample}}
%
%\newenvironment{GrayExercise}[1][]{% Deprecated.
%	\ifx&#1&\begin{grayexercise}\else\begin{grayexercise}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{grayexercise}
%}
%
%\newenvironment{GrayExerciseL}[2][]{
%	\ifx&#1&\begin{grayexercise}\else\begin{grayexercise}[#1]\fi
%	\label{#2}
%	\glossary{\textbf{Exercise \ref{#2}}}
%	}{\end{grayexercise}}
%
%\newenvironment{GrayTheorem}[1][]{% Deprecated.
%	\ifx&#1&\begin{graytheorem}\else\begin{graytheorem}[#1]\fi\textbf{Deprecated: Use L-version. CCM 190803.}}
%	{\end{graytheorem}}
%
%\newenvironment{GrayTheoremL}[2][]{
%		\global\NeedQEDtrue
%		\ifx&#1&\begin{graytheorem}\else\begin{graytheorem}[#1]\fi
%		\label{#2}
%		\glossary{\textbf{Theorem \ref{#2}}}
%	}
%	{\ifNeedQED\relax\else\relax\fi\global\NeedQEDfalse\end{graytheorem}
%}
%
%% GrayProof's are -outside- the theorem etc, and so need their \qed's.
%\newenvironment{GrayProof}{\begin{proof}}{\qed\end{proof}}
%
%% In case we want a uniform change.
%%\newenvironment{Figure}[2] {\begin{figure}[t]\def\z{#1}\def\zz{#2}\small}{\caption{\zz\quad \hrulefill}\label{\z}\end{figure}}
%%\newenvironment{Figure}[2] {\begin{figure}[t]\def\z{#1}\def\zz{#2}\small}{\caption{\zz\quad \raisebox{.2em}{\rule{2em}{.05em}} }\label{\z}\end{figure}}
%%\newenvironment{Figure}[2] {\begin{figure}\def\z{#1}\def\zz{#2}\small}{\caption{\makebox[0em][r]{\raisebox{.2em}{\rule{2em}{.05em}}\hspace{5.5em}}\quad\zz\quad\raisebox{.2em}{\rule{2em}{.05em}}}\label{\z}\end{figure}}
%
%\newcommand\Chapter[1]{\chapter{#1}}
%\newcommand\Section[1]{\section{#1}}
%\newcommand\Subsection[1]{\subsection{#1}}
%\newcommand\Subsubsection[1]{\subsubsection{#1}}
%
%\newcounter{Enums}			% For run-on enumerations.
%\newcounter{enumSaver}		% Another one: rationalise them at some point.
%
%% \Footnote[]{xxx} closes up 0.1em.
%% \Footnote{xxx} is as normal..
%% \Footnote[<length>]{xxx} closes up <length>.
%% http://tex.stackexchange.com/questions/127502/difference-between-if-and-ifx
%\newcommand\Footnote[2][\empty] {\ifx#1\empty\kern-0.1em\else\if*#1\relax\else\kern-#1\fi\fi\footnote{#2}} 
%
%% Helpers for referring to them.
%\newcommand\Cor[1] {Cor.~\ref{#1}}
%\newcommand\Chp[1] {Chap.~\ref{#1}}
%\newcommand\Def[1] {Def.~\ref{#1}}
%\newcommand\Ex[1]  {Exercise~\ref{#1}}
%\newcommand\Eg[1]  {Example~\ref{#1}}
%\newcommand\EqRef[1] {\Eqn{#1}} % Replace this by \Eqn everywhere.
%\newcommand\Itms[2] {(\ref{#1}--\ref{#2})}
%\newcommand\Lem[1] {Lem.~\ref{#1}}
%\newcommand\Note[1] {\FnSym\ref{#1}}
%\newcommand\NOTE[1] {\Note{#1} on \Pg{#1}}
%\newcommand\Prt[1] {Part~\ref{#1}}
%\newcommand\Pg[1] {p.~\pageref{#1}}
%\newcommand\Thm[1] {Thm.~\ref{#1}}
%\newcommand\Prop[1] {Prop.~\ref{#1}}
%\newcommand\Prog[1] {Prog.~(\ref{#1})} % Prog already used; but we will get rid of it eventually, using ProgMini instead.
%% Following for beginning-of-sentence instances.
%\newcommand\COR[1] {Corollary~\ref{#1}}
%\newcommand\CHP[1] {Chapter~\ref{#1}}
%\newcommand\DEF[1] {Definition~\ref{#1}}
%\newcommand\EX[1]  {Exercise~\ref{#1}}
%\newcommand\EG[1]  {Example~\ref{#1}} % How should we distinguish \Ex and \Eg?
%\newcommand\EQN[1] {Equation (\ref{#1})}
%\newcommand\FIG[2][\empty] {\ifx#1\empty Figure~\ref{#2}\else Figure~\ref{#2}(#1)\fi}
%\newcommand\ITM[1] {Item (\ref{#1})}
%\newcommand\ITMS[2] {Items (\ref{#1}--\ref{#2})}
%\newcommand\LEM[1] {Lemma~\ref{#1}}
%\newcommand\PRT[1] {Part~\ref{#1}}
%\newcommand\PG[1] {Page~\pageref{#1}}
%\newcommand\SEC[1] {Section~\ref{#1}}
%\newcommand\THM[1] {Theorem~\ref{#1}}
%\newcommand\PROP[1] {Proposition~\ref{#1}}
%
%%
%% Proof -- is it a part of the theorem, or not?
%% That is, do we write
%%
%%Theorem
%%	statement of theorem
%%END_THEOREM
%%Proof
%%	details of proof
%%END_PROOF
%%
%% or do we write
%%
%%Theorem
%%	statement of theorem
%%Proof
%%	details of proof
%%END_MATHS
%%
%%\newcommand\Proof{\par\noindent\textit{Proof:}\quad}
%
%% Same for "Proof", most places use "proof" so I made them synonyms (just with \qed in the
%% end) for consistency. We can easily change "proof" if needed.
%% Kostas 180506
%%\newenvironment{Proof}{\begin{proof}}{\qed\end{proof}}
%% \newenvironment{Proof}{\par\noindent\textbf{Proof}\quad}{}%~\hfill$\Box$}
%
%% push \qed to the right
%\renewcommand{\qed}{\ensuremath{\hfill\qedsymbol}}
%
%%%% 0923: Environments for typesetting ASCII text and program text
%%
%
%% See http://tex.stackexchange.com/questions/11973/verbatim-environment-and-line-breaking
%\lstnewenvironment{ProgDeprecated} {
%	\lstset{
%		language=csh,
%		basicstyle=\ttfamily,	% 1350: Should agree with \PF, i.e. program font.
%		breaklines=false,	% 0922: Don't wrap lines in Prog.
%		showspaces=false,
%		keywords={vis,hid,var,while,if,end,begin,to,then,fi,skip},
%		columns=flexible,
%		escapechar=\%,	% 0920: Use "%" for escape to LaTeX, since it doesn't work as comment in verbatim anyway.
%		mathescape=true
%	}
%}{}
%
%\newenvironment{ProgFrags}{ % For inline program fragments, delimited both sides by "!" .
%	\lstMakeShortInline[
%		language=csh,
%		basicstyle=\ttfamily,	% 1350.
%		breaklines=false,	% 0922.
%		showspaces=false,
%		keywords={vis,hid,var,while,if,end,begin,to,then,fi,skip},
%		columns=flexible,
%		escapechar=\%,	% 0920. But doesn't work in-line?
%		mathescape=true
%	]!
%}
%{\lstDeleteShortInline!}
%
%\lstnewenvironment{ASCII} {
%	\lstset{
%		language=csh,
%		basicstyle=\ttfamily,
%		showspaces=false,
%		breaklines=true,	% 0922: Wrap lines in ASCII.
%		breakindent=0pt,
%		keywords={},
%		columns=flexible,
%		escapechar=\%,	% 0920.
%		mathescape=true
%	}
%}{}
%
%\newenvironment{EqnText}[1] {\begin{equation}\label{#1}\begin{minipage}{0.8\linewidth}}{\end{minipage}\end{equation}}
%
%
%%%% Here's two toy examples: the first creates a "quote like" display, with no number and therefore no way of referring to it. The second makes an "equation like" display, with a label.
%
%% Inside "Prog" you can escape to LeTeX with %stuff% and escape to maths with $maths$. Obviously "%" doesn't work as comment in that case.
%
%% No number, no label.
%%	\newcommand\Leak {print} % We have't decided whether to call it "leak", or "print" or "reveal".
%%	\begin{ProgDeprecated}
%%	x:= 0;
%%	y:= 1 $\PC{\nicefrac{1}{2}}$ 2;
%%	if x=0 then
%%		while y=2 do
%%			%\Leak% 0 ${\ND}$ (x+y)
%%		end
%%	fi
%%	\end{ProgDeprecated}
%
%% With number and label. Unfortunately, I cannot manage to combine the \begin{EqnText}\begin{ProgDeprecated} into a single \begin{Something}.
%% On the other hand, EqnText can be used more generally when you want an equation-like reference to something that isn't maths:
%% it doesn't have to have Prog inside.
%
%%	\begin{EqnText}{e1234}
%%	\begin{ProgDeprecated}
%%	x:= 0;
%%	y:= 1 $\PC{\nicefrac{1}{2}}$ 2;
%%	if x=0 then
%%		while y=2 do
%%			%\Leak% 0 ${\ND}$ (x+y)
%%		end
%%	fi
%%	\end{ProgDeprecated}
%%	\end{EqnText}
%
%
%%%% Macros for equational reasoning
%%
% For reasoning about program texts.
%
%
%%%% Here's a toy example:
%
%%	\begin{Reason}
%%	\Step{}{ % First step has no operator and no reason.
%% 		first expression
%%	}
%%	\StepR{$=$}{because it's equal}{ % Second step is related to first by =, and has a reason. Note $$.
%% 		second expression
%%	}
%%	\Space % Blank line before and after multi-line steps: this one's before.
%% 	% Third step is related to second by if, and has a long reason. Not no $$.
%%	\WideStepR{$=$}{because it's equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, }{
%% 		third expression
%%	}
%%	\Space % This one's after.
%%	\Step{$\Implies$}{ % Last step ends with $\quad$ and some punctuation, if it makes sense grammatically
%% 		fourth expression \quad.
%%	}
%%	\end{Reason}
%
%%%% Here's a real example from CSF14 p10.
%% 	Note there's no colon before, and a comma afterwards. The grammar is thus the same as if we had written
%%
%%	Thus we calculate $(x+1)^2=x^2+2x+1$, whence the result follows...
%%
%%
%
%%	Thus we calculate
%%	\begin{Reason}
%%	\Step{}{
%%		\WDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}} 
%%	}
%%	\StepR{$=$}{$d$ is underlying metric; \Def{d0636}}{
%% 		\min_{S\In\Spc{S}_{\Sigma,\Tau}} \Expec{S}{d}
%%	}
%%	\StepR{$=$}{take unique $S$ in $\Spc{S}$ as at \Eqn{e1314}}{
%% 		\Expec{S}{d}
%%	}
%%	\Space
%%	\StepR{$=$}{define $d_\sigma(\tau)\Defs d(\sigma,\tau)$ to allow Currying;\\
%%            $S$ at \Eqn{e1314} has point left-marginal $\Point{\pi}$}{
%% 		\Expec{\ChanHyp{\pi}{{C}}}{d_\pi}
%%	}
%%	\Space
%%	\StepR{$=$}{define $g$ so that $\GVul{\Point{\tau}}{g} = d_\pi(\tau){+}1$; see below}{
%%		\GVul{\ChanHyp{\pi}{{C}}}{g} - 1
%%	}
%%	\StepR{$=$}{$\GVul{\Point{\pi}}{g} = d_\pi(\pi){+}1 = 1$}{
%%		\GVul{\ChanHyp{\pi}{{C}}}{g} - \GVul{\Point{\pi}}{g}
%%	}
%%	\StepR{$\leq$}{\Def{d0730}}{
%%		\ACapty{{C}}{\AllPi}{\pi}
%%	}
%%	\StepR{$\leq$}{\Lem{l1411}}{
%%		\KDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}} ~,
%%	}
%%	\end{Reason}
%%	whence the result follows because we have sandwiched $\ACapty{{C}}{\AllPi}{\pi}$
%%	between $\WDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}}$
%%	and $\KDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}}$
%%	--- which from \Thm{t0647} are equal.
%
%% For giving an equation number to something that's not just maths.
%\newenvironment{NumMini}[1]{\begin{equation}\label{#1}\begin{minipage}{.8\linewidth}}{\end{minipage}\end{equation}}
%
%

